How Propense Are Large Language Models at Producing Code Smells? A Benchmarking Study

Large Language Models (LLMs) have shown significant potential in automating software engineering tasks, particularly in code generation. However, current evaluation benchmarks, which primarily focus on accuracy, fall short in assessing the quality of the code generated by these models, specifically their tendency to produce code smells. To address this limitation, we introduce CodeSmellEval, a benchmark designed to evaluate the propensity of LLMs for generating code smells. Our benchmark includes a novel metric: Propensity Smelly Score (PSC), and a curated dataset of method-level code smells: CodeSmellData. To demonstrate the use of CodeSmellEval, we conducted a case study with two state-of-the-art LLMs, CodeLlama and Mistral. The results reveal that both models tend to generate code smells, such as simplifiable-condition and consider-merging-isinstance. These findings highlight the effectiveness of our benchmark in evaluating LLMs, providing valuable insights into their reliability and their propensity to introduce code smells in code generation tasks.

==> sections/6_acknowledgments.tex <==
\section{Acknowledgments}
\label{sec:acknowledgments}

This research has been supported in part by the NSF CCF-2311469, CNS-2132281, CCF-2007246, and CCF-1955853. We also acknowledge support from Cisco Systems. Any opinions, findings, and conclusions expressed herein are the authors’ and do not necessarily reflect those of the sponsors.

==> sections/old/3_approach.tex <==
\section{Code Smells Evaluation}
\label{sec:approach}
We rely on \astscore \REF to estimate the propensity of an \llm in introducing code smells during code generation tasks. In this section, we introduce this interpretability metric and explain how it is applied to address \ref{rq:code_smells} and \ref{rq:model_comparison}.

%%%% Overview of ASTScore
\textbf{Using logit probabilities.} \astscore is a post-hoc interpretability metric, calculated by extracting the non-normalized log-probabilities (logits) for each token prediction from the last hidden layer of a decoder-based transformer (\eg GPT). The softmax function ($\sigma$) is applied to these logits to estimate the probabilities of the expected tokens in a sequence. For a token $w_i = t, t \in V$, the probability $P(w_i = t | w_{<i})$ is computed as shown in \equref{eq:prob_computation}, where $w_{i,t}$ is the logit for the expected token $t$ at position $i$, $V$ is the vocabulary, and the denominator is the sum of exponentiated logits across all vocabulary tokens, normalizing the probabilities. The computation of $\sigma(z_i)_t$ is influenced by the preceding context, as decoder-based models are auto-regressive.

\vspace{-0.1em}
\begin{equation}
    \label{eq:prob_computation}
    P(w_i = t | w_{<i}) \approx \sigma(z_i)_t = \frac{e^{z_{i,t}}}{\sum_{j=1}^{|V|}{e^{z_{i,j}}}}
\end{equation}


%%%% Aggregation Function
\textbf{Meaningful Structures $\mathbb{M}$.} Using an alignment function ($\delta$), tokens $w_i \in s$ are grouped into a meaningful structure $\mu \in \mathbb{M}$. An aggregation function ($\theta$) is then applied to compute a central tendency statistic (\eg median, mean) of their probabilities, providing an overall probability estimate for predicting $\mu$. Once $P(w_i | w_{<i})$ is computed, the probability of each token’s predicted value is treated independently to calculate the overall estimate of $\mu$. The \astscore computation for a meaningful concept $\mu$ is shown in \equref{eq:score_computation}.

\vspace{-0.1em}
\begin{equation}
\label{eq:score_computation}
    %P(\mu) = \theta_\mu(s) = \frac{1}{n} \sum_{i=1}^{n} P(w_i | w_{<i}), w \in \delta_\mu(s)
    P(\mu) = \theta_\mu(s) =  Median[P(w_i | w_{<i})], w \in \delta_\mu(s)
\end{equation}

Figure \REF illustrates an example of computing \astscore for a Python snippet containing the code smell: \textit{inconsistent-return-statements}. 

%%%% Definition of Meaningful Structures. 
\textbf{Code Smells} The definition of the set of meaningful structures $T$ used in function $\delta$ depends on the problem context. For example, token probabilities can be aggregated using syntax-based decomposition, based on elements defined by the grammar of a programming language (\eg identifiers, conditionals, statements). In this paper, we propose defining the set of concepts $T$ using types of code smells. Figure \REF illustrates the full taxonomy of code smells in $T$ evaluated in our case study.

%%%%% Global Estimates
\textbf{Global Estimates.} Lastly, the average of \equref{eq:score_computation} for a given code smell type ($\mu$) is computed across all code snippets $s$ in a dataset to estimate the overall propensity of code smells being generated by an \llm. We use this estimate to answer \ref{rq:code_smells}. Additionally, to compare the probability distributions between the selected models and answer \ref{rq:model_comparison}, we compute the overlapping and confidence intervals on the bootstrapped distributions. 

\ALEJO{TODO: Complement this part explaining the difference of local vs global and the definition of propensity. }



\label{sec:approach}

==> sections/old/4_results_discussion.tex <==
\section{Results \& Discussion}
\label{sec:results_discussion}

In this section, we presents the results of our case study addressing  \ref{rq:code_smells} and \ref{rq:model_comparison}. 

%%%%%%%% RESULTS TABLE 
\input{tables/results}
%%%%%%%%%%%%%%%%%%%%%%

\subsection{\ref{rq:code_smells} Propensity of Code Smell generation}
\tabref{tab:results} presents the probability scores computed for each code smell using both M1 and M2. Considerably, $17$ out of $20$ code smells have a probability higher than the propensity threshold of $0.5$, indicating that both models are prone to generating these smells. Specifically, the top five smells with the highest probabilities in both models are nested-min-max (W3301), simplifiable-condition (R1726), consider-merging-isinstance (R1701), comparison-with-itself (R0124), and chained-comparison (R1716).


%%%%%%% Distributions for RQ1
\begin{figure*}[ht]
		\centering
  \vspace{-1em}
  \includegraphics[width=1\textwidth]{images/result_distributions.pdf}
		\caption{Boxplots showing the probability distributions of code smells, with 100 instances per sample. The red line at $0.5$ indicates the propensity threshold.}
    \label{fig:boxplots}
    \vspace{-1em}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht]
		\centering
  \vspace{-1em}
  \includegraphics[width=1\textwidth]{images/result_distribution_comparison.pdf}
		\caption{Comparison of distribution between M1 and M2 for the type of code smells with the highest differences between means}
    \label{fig:dist_comparison}
    \vspace{-1em}
\end{figure*}

==> sections/old/related_work.tex <==
%RobustAPI~\cite{zhong_can_2024} evaluates the robustness and reliability of LLM-generated code by examining common API misuse patterns \DANIEL{@ALIF I dont get this}.

%\ALIF{Detection rules such as different object-oriented metrics with predefined threshold values can be modified with ~\cite{arcelli_fontana_automatic_2015}data-driven methods to automatically derive threshold values for code metrics to implement detection rules for code smells detection.}

%\llms have demonstrated impressive capabilities in automating software engineering tasks like code generation \cite{lin_when_2024, cambon_early_2023}, significantly enhancing productivity \cite{cambon_early_2023}. However, since they are trained on publicly available repositories \cite{mohsin_can_2024, hajipour_codelmsec_2024}, the code they generate can contain vulnerabilities and code smells, which may propagate to production code \cite{mohsin_can_2024, hajipour_codelmsec_2024, siddiq_sallm_2024, kaniewski_vulnerability_2024}. Code smells often indicate deeper issues in the codebase, affecting both code quality and performance as it becomes more complex\cite{mahalakshmi_code_2023, siksna_machine_2023}. For instance, a case study of ChatGPT and Copilot for code generation~\cite{sagodi_methodology_2024} found that human expertise is essential to ensure the correctness of the code and remove code smells \cite{tosi_studying_2024}. 

%With the emergence of \llms, frameworks like LCG \cite{lin_when_2024}, iSmell \cite{di_wu_ismell_2024}, and PromptSmell \cite{liu_prompt_2024} explored a combination of \llms agents, prompting techniques such in-context learning (ICL) and chain-of-thought (CoT)~\cite{kaniewski_vulnerability_2024}, and prompt learning to automatically detect and mitigate multi-label code smells in code generation. Copilot-in-the-loop \cite{zhang_copilot---loop_2024} study found that Copilot can detect $8$ out of $10$ types of code smells generated by Github Copilot, among which Multiply-Nested Container is the most common one. 





%\ALIF{ \llms have demonstrate an impressive ability in automating software engineering tasks like code generation~\cite{lin_when_2024},~\cite{cambon_early_2023}, enhancing productivity~\cite{cambon_early_2023}. Since they are trained on publicly available repositories~\cite{mohsin_can_2024},~\cite{hajipour_codelmsec_2024}, the code they generate contains vulnerabilities and code smells. As a result, these code smells can propagate to production code~\cite{mohsin_can_2024},~\cite{hajipour_codelmsec_2024},~\cite{siddiq_sallm_2024},~\cite{kaniewski_vulnerability_2024}. Code smells indicate deeper problems in the codebase that affect the code quality and performance~\cite{mahalakshmi_code_2023},~\cite{siksna_machine_2023} as the project grows complex~\cite{siksna_machine_2023}. A case study of ChatGPT and Copilot for code generation~\cite{sagodi_methodology_2024} revealed that human expertise~\cite{tosi_studying_2024} is required to ensure code with correctness and free of code smells. To detect these code smells, many studies explored approaches like metric, heuristic, machine learning and deep learning based techniques~\cite{li_multi-label_2022}, some even combining~\cite{mahalakshmi_code_2023} these techniques to improve the detection. While these approaches work well for individualized code smells like Data Class, God Class, Feature Envy and Long Method~\cite{mahalakshmi_code_2023},~\cite{mahalakshmi_code_2023},~\cite{skipina_automatic_2024}, they fail to detect smells in complex applications~\cite{siksna_machine_2023}. With the emergence of LLMs, frameworks like LCG~\cite{lin_when_2024}, iSmell~\cite{di_wu_ismell_2024}, and PromptSmell ~\cite{liu_prompt_2024} explored mixture of LLM agents, prompting techniques like in-context learning (ICL) and chain-of-thought (CoT)~\cite{kaniewski_vulnerability_2024} and prompt learning to automatically detect and mitigate multi-label code smells in code generation. Copilot-in-the-loop~\cite{zhang_copilot---loop_2024} study found that Copilot can detect 8 out of 10 types of code smells generated by Github Copilot, among which Multiply-Nested Container is the most common one. 
\\
%Existing benchmarks and datasets primarily focus on functional correctness~\cite{siddiq_sallm_2024} of the generated code, but do not take into account confounding variables that affect the quality of the code. But manually annotated datasets like DACOS~\cite{nandani_dacosmanually_2023} and DACOSX~\cite{nandani_dacosmanually_2023} attempts to aid context-aware machine-learning models to detect code smells at three different granular levels- multifaceted abstraction, complex method and long parameter list which contains 5,192 code snippets with 10,267 annotations. CodeLMSec~\cite{hajipour_codelmsec_2024} attempts to benchmark code generation models’ susceptibility to generating vulnerable code using few-shot prompting. Similarly, RobustAPI~\cite{zhong_can_2024} dataset evaluates the robustness and reliability of LLM-generated code by examining common API misuse patterns that 62\% of generated code contained API misuses, which could lead to unforeseen consequences. SALLM~\cite{siddiq_sallm_2024} also benchmarks LLM’s ability to generate secure code by providing a dataset of secure Python prompts and novel metrics for evaluating the security of the generated code.
%\\ \DANIEL{All of this goes into the intro}
%While most of the recent studies explored various prompting techniques~\cite{kaniewski_vulnerability_2024} and prompting based benchmarks ~\cite{hajipour_codelmsec_2024},~\cite{siddiq_sallm_2024},~\cite{yang_dlap_2024} to detect and mitigate code smells~\cite{dinh_large_2023} in code generation, static analysis tools, such as linters~\cite{siddiq_empirical_2022},~\cite{ding_static_2023} have been underexplored to detect code smells. There is also a lack of interpretability metrics~\cite{rodriguez-cardenas_benchmarking_2023},~\cite{nader_palacio_toward_2024} to assess code quality in black box code generation models. Existing studies mostly focus on accuracy and vulnerabilities but fail to measure the propensity to which LLMs generate code smells. We aim to address this gap by implementing ASTScore (a post-hoc interpretability metric) to evaluate the propensity of LLM models to generate code smells with a curated dataset of pylint code smells for future studies to better understand the LLM code generation process.}

==> tables/models.tex <==
\begin{table}[]

\centering
\caption{Evaluated Decoder-Based Transformers.}
\label{tab:models}
\vspace{-0.5em}
\scalebox{0.9}{

\setlength{\tabcolsep}{4pt} 

%%%%%%%%%%%% TABLE
\begin{tabular}{lllllll}
\hline
\textbf{ID} &
   &
  \textbf{Model} &
  \textbf{Size} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Hidden \\ Layers\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Attention \\ Heads\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Vocabulary\\ Size\end{tabular}} \\ \hline
M1 &
   &
  CodeLlama-7b-Instruct-hf \cite{roziere_code_2024} &
  7B &
  32 &
  32 &
  32016 \\
M2 &
   &
  Mistral-7B-v0.3 \cite{jiang_mistral_2023} &
  7B &
  32 &
  32 &
  32768 \\ \hline
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%
} % % End Scalebox
\vspace{-1em}
\end{table}

==> tables/results.tex <==
\begin{table}[]
\centering
\caption{Obtained results of probability scores for each type of code smell. (\textbf{bold}:strong difference between distributions, background:smells under the propensity threshold)}
\label{tab:results}
\vspace{-0.5em}
\scalebox{0.87}{

\setlength{\tabcolsep}{4pt} 
%%%%%%%%%%%% TABLE
\begin{tabular}{lllllllllc}
 &
  \multicolumn{3}{c}{\textit{\begin{tabular}[c]{@{}c@{}}M1\cite{roziere_code_2024}\end{tabular}}} &
   &
  \multicolumn{3}{c}{\textit{\begin{tabular}[c]{@{}c@{}}M2\cite{jiang_mistral_2023}\end{tabular}}} &
   &
  \multicolumn{1}{l}{} \\
\multicolumn{1}{c}{\textbf{Code Smell}} &
  \multicolumn{1}{c}{\textbf{mean}} &
  \multicolumn{1}{c}{\textbf{std}} &
  \multicolumn{1}{c}{\textbf{iqr}} &
   &
  \multicolumn{1}{c}{\textbf{mean}} &
  \multicolumn{1}{c}{\textbf{std}} &
  \multicolumn{1}{c}{\textbf{iqr}} &
   &
  \textbf{$\nabla$mean [CI]} \\ \hline
\textbf{W0150} & \textbf{0.704} & \textbf{0.1591} & \textbf{0.119} & \textbf{} & \textbf{0.610} & \textbf{0.143} & \textbf{0.087} & \textbf{} & \textbf{0.094 $\pm$ 0.042} \\
\textbf{R1726} & \textbf{0.889} & \textbf{0.029}  & \textbf{0.043} & \textbf{} & \textbf{0.816} & \textbf{0.017} & \textbf{0.038} & \textbf{} & \textbf{0.071 $\pm$ 0.006} \\
\textbf{R0123} & \textbf{0.734} & \textbf{0.041}  & \textbf{0.047} & \textbf{} & \textbf{0.662} & \textbf{0.043} & \textbf{0.046} & \textbf{} & \textbf{0.072 $\pm$ 0.012} \\
\textbf{C0103} & \textbf{0.648} & \textbf{0.213}  & \textbf{0.325} & \textbf{} & \textbf{0.580} & \textbf{0.212} & \textbf{0.308} & \textbf{} & \textbf{0.068 $\pm$ 0.059} \\
\textbf{R0124} & \textbf{0.822} & \textbf{0.059}  & \textbf{0.047} & \textbf{} & \textbf{0.765} & \textbf{0.065} & \textbf{0.058} & \textbf{} & \textbf{0.057 $\pm$ 0.017} \\
W0101          & 0.608          & 0.103           & 0.053          &           & 0.563          & 0.093          & 0.067          &           & 0.045 $\pm$ 0.027          \\
\rowcolor[HTML]{EFEFEF} 
C2401          & 0.246          & 0.078           & 0.061          &           & 0.204          & 0.051          & 0.028          &           & 0.042 $\pm$ 0.018          \\
R1716          & 0.808          & 0.098           & 0.1            &           & 0.767          & 0.107          & 0.097          &           & 0.040 $\pm$ 0.028          \\
C3001          & 0.618          & 0.144           & 0.170          &           & 0.579          & 0.155          & 0.189          &           & 0.038 $\pm$ 0.041          \\
R1701          & 0.827          & 0.089           & 0.092          &           & 0.789          & 0.100          & 0.104          &           & 0.037 $\pm$ 0.026          \\
W0108          & 0.724          & 0.152           & 0.191          &           & 0.688          & 0.157          & 0.182          &           & 0.036 $\pm$ 0.043          \\
\rowcolor[HTML]{EFEFEF} 
R0913          & 0.386          & 0.116           & 0.167          &           & 0.356          & 0.111          & 0.153          &           & 0.031 $\pm$ 0.031          \\
R0916          & 0.736          & 0.062           & 0.04           &           & 0.710          & 0.064          & 0.054          &           & 0.026 $\pm$ 0.017          \\
\rowcolor[HTML]{EFEFEF} 
C0104          & 0.462          & 0.248           & 0.403          &           & 0.440          & 0.236          & 0.318          &           & 0.022 $\pm$ 0.067          \\
W0718          & 0.775          & 0.121           & 0.167          &           & 0.758          & 0.113          & 0.155          &           & 0.016 $\pm$ 0.032          \\
R1702          & 0.770          & 0.054           & 0.029          &           & 0.755          & 0.056          & 0.033          &           & 0.015 $\pm$ 0.015          \\
W3301          & 0.894          & 0.036           & 0.075          &           & 0.884          & 0.029          & 0.039          &           & 0.009 $\pm$ 0.009          \\
W0130          & 0.691          & 0.080           & 0.112          &           & 0.686          & 0.069          & 0.070          &           & 0.005 $\pm$ 0.020          \\
W0719          & 0.520          & 0.200           & 0.291          &           & 0.535          & 0.229          & 0.332          &           & -0.014 $\pm$ 0.059         \\
C0121          & 0.696          & 0.161           & 0.224          &           & 0.738          & 0.191          & 0.277          &           & -0.042 $\pm$ 0.049         \\ \hline
\end{tabular}

%%%%%%%%%%%%%%%%%%%%%%%
} % % End Scalebox
\caption*{\small{*Each code smell has a sample size of 100}}
\vspace{-1em}
\end{table}
